Lookback for Learning to Branch

The expressive and computationally inexpensive bipartite Graph Neural Networks (GNN) have been shown to be an important component of deep learning based Mixed-Integer Linear Program (MILP) solvers. Recent works have demonstrated the effectiveness of such GNNs in replacing the branching (variable selection) heuristic in branch-and-bound (B&B) solvers. These GNNs are trained, offline and on a collection of MILPs, to imitate a very good but computationally expensive branching heuristic, strong branching. Given that B&B results in a tree of sub-MILPs, we ask (a) whether there are strong dependencies exhibited by the target heuristic among the neighboring nodes of the B&B tree, and (b) if so, whether we can incorporate them in our training procedure. Specifically, we find that with the strong branching heuristic, a child node's best choice was often the parent's second-best choice. We call this the "lookback" phenomenon. Surprisingly, the typical branching GNN of Gasse et al. (2019) often misses this simple "answer". To imitate the target behavior more closely by incorporating the lookback phenomenon in GNNs, we propose two methods: (a) target smoothing for the standard cross-entropy loss function, and (b) adding a Parent-as-Target (PAT) Lookback regularizer term. Finally, we propose a model selection framework to incorporate harder-to-formulate objectives such as solving time in the final models. Through extensive experimentation on standard benchmark instances, we show that our proposal results in up to 22% decrease in the size of the B&B tree and up to 15% improvement in the solving times.

==> inputs/big-evaluation-side.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{wraptable}{r}{0.80\textwidth}
% \vspace{-5pt}
\captionsetup{justification=centering}
\scriptsize
\caption{
Performance of \textit{branching strategies} on \textit{big} evaluation instances. Refer to section~\ref{sec:experiments} for more details. Time (c) and Node (c) represent the 1-shifted geometric mean of respective measures on the instances commonly solved by all the branching strategies. The best performing numbers are in \textbf{bold}.}
\label{tab:big-evaluation}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{8pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=3.0]@{\hspace{3pt}}
    S[table-format=4.0]@{}
%
    }
    \toprule

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Time (c)} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes (c)} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{fsb}
        &  2075.60   & 1643.78  &    0 & 53 &   336 \\
        
    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  202.78   & 113.47 &    1 & 100 &   4640 \\

    \textsc{tunedRPB}
        &  205.57   & 112.80 &    0 & 100 &   4611 \\
        
    \textsc{gnn}
        & \B 139.30   & \B 72.17 &   \B 64 & 100 &   4142 \\
    \textsc{gnn-PAT} (ours)
        &  141.63  & 73.31  &    35 & 100 &   \B 3754 \\

    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Combinatorial Auction} \\
    \\[-3pt]

    \cmidrule(lr){1-6} 

    \textsc{fsb}
        & 2700  & n/a  &    0 & 0 &   n/a \\

    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  1883.32   &  1213.57 &  1 & 47 &   58766 \\

    \textsc{tunedRPB}
        &  1851.83   &  1168.58  & 0 & 48 &   58155 \\

    \textsc{gnn}
        &  1708.99   &  991.07   & 5 & 54 &   39535 \\

    \textsc{gnn-PAT} (ours)
        & \B 1601.28   & \B 892.85 &   \B 54 & \B 59 &  \B 38385  \\
       
    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Set Covering} \\
    \\[-3pt]

    \cmidrule(lr){1-6} 

    \textsc{fsb}
        & 917.39  & 758.19  &    8 & 85 &   50 \\

    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  737.66   & 607.19 &    3 & 92 &   104 \\

    \textsc{tunedRPB}
        &  751.27   & 619.27  &    2 & 92 &  \B 97 \\
        
    \textsc{gnn}
        &   646.03    & 525.80 &    16 & 92 &    293 \\

    \textsc{gnn-PAT} (ours)
        & \B  581.91  & \B 471.20  &  \B 66 & \B 95 &   304 \\

    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Capacitated Facility Location} \\
    \\[-3pt]

    \cmidrule(lr){1-6}
    
    \textsc{fsb}
        & 2700  & n/a  &    0 & 0 &   n/a \\
    \cmidrule(lr){1-6} 

    \textsc{rpb}
        & 1984.91   &  888.04 &    0 & 32 &   12407 \\

    \textsc{tunedRPB}
        & 2016.85   &  952.25  &    0 & 33 &   12940 \\
        
    \textsc{gnn}
        &  1207.62  &  279.71 &    14 & 65 &   7934 \\

    \textsc{gnn-PAT} (ours)
        &  \B 1035.32  & \B 233.97 &  \B  56 & \B  70 & \B  6122 \\
        
    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Maximum Independent Set} \\
    \\[-3pt]
    \bottomrule
\end{tabular}
% \vspace{-15pt}
\end{wraptable}


==> inputs/big-evaluation.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[t]
\caption{
Performance of \textit{branching strategies} on \textit{big} evaluation instances. Refer to section~\ref{sec:experiments} for more details. Time (c) and Node (c) represent the 1-shifted geometric mean of respective measures on the instances commonly solved by all the branching strategies. The best performing numbers are in \textbf{bold}.}
\label{tab:big-evaluation}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{8pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=3.0]@{\hspace{3pt}}
    S[table-format=4.0]@{}
%
    }
    \toprule

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Time (c)} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes (c)} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{fsb}
        &  2075.60   & 1643.78  &    0 & 53 &   336 \\
        
    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  202.78   & 113.47 &    1 & 100 &   4640 \\

    \textsc{tunedRPB}
        &  205.57   & 112.80 &    0 & 100 &   4611 \\
        
    \textsc{gnn}
        & \B 139.30   & \B 72.17 &   \B 64 & 100 &   4142 \\
    \textsc{gnn-PAT} (ours)
        &  141.63  & 73.31  &    35 & 100 &   \B 3754 \\

    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Combinatorial Auction} \\
    \\[-3pt]

    \cmidrule(lr){1-6} 

    \textsc{fsb}
        & 2700  & n/a  &    0 & 0 &   n/a \\

    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  1883.32   &  1213.57 &  1 & 47 &   58766 \\

    \textsc{tunedRPB}
        &  1851.83   &  1168.58  & 0 & 48 &   58155 \\

    \textsc{gnn}
        &  1708.99   &  991.07   & 5 & 54 &   39535 \\

    \textsc{gnn-PAT} (ours)
        & \B 1601.28   & \B 892.85 &   \B 54 & \B 59 &  \B 38385  \\
       
    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Set Covering} \\
    \\[-3pt]

    \cmidrule(lr){1-6} 

    \textsc{fsb}
        & 917.39  & 758.19  &    8 & 85 &   50 \\

    \cmidrule(lr){1-6} 

    \textsc{rpb}
        &  737.66   & 607.19 &    3 & 92 &   104 \\

    \textsc{tunedRPB}
        &  751.27   & 619.27  &    2 & 92 &  \B 97 \\
        
    \textsc{gnn}
        &   646.03    & 525.80 &    16 & 92 &    293 \\

    \textsc{gnn-PAT} (ours)
        & \B  581.91  & \B 471.20  &  \B 66 & \B 95 &   304 \\

    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Capacitated Facility Location} \\
    \\[-3pt]

    \cmidrule(lr){1-6}
    
    \textsc{fsb}
        & 2700  & n/a  &    0 & 0 &   n/a \\
    \cmidrule(lr){1-6} 

    \textsc{rpb}
        & 1984.91   &  888.04 &    0 & 32 &   12407 \\

    \textsc{tunedRPB}
        & 2016.85   &  952.25  &    0 & 33 &   12940 \\
        
    \textsc{gnn}
        &  1207.62  &  279.71 &    14 & 65 &   7934 \\

    \textsc{gnn-PAT} (ours)
        &  \B 1035.32  & \B 233.97 &  \B  56 & \B  70 & \B  6122 \\
        
    \cmidrule(lr){1-6} 
    \\[-7pt]
    & \multicolumn{5}{ c }{Maximum Independent Set} \\
    \\[-3pt]
    \bottomrule
\end{tabular}
\vspace{-15pt}
\end{table}


==> inputs/big-results.tex <==
\begin{table}[htp]
    \centering
    \begin{tabular}{p{25mm}|ccc}
    \toprule
    {} & \multicolumn{3}{c}{big} \\
    {} & \multicolumn{2}{c}{Time} &  Nodes \\
    {} &       GM &     Wins &     GM \\
    \midrule
    FSB   &   2075.60 &    0/ 53 &    336 \\
    \midrule
    RPB  &    202.78 &    0/100 &   4640 \\
    TunedRPB-t  &  205.57 &    0/100 &   4611 \\
    GNN &   139.30 &   16/100 &   4142 \\
    GNN-PAT &      \textbf{126.50} &   \textbf{84}/100 &   \textbf{3904} \\
    \bottomrule
    \multicolumn{3}{ c }{Combinatorial Auctions} \\
    
    \midrule
    FSB  &    2700.00 &    0/  0 &     nan \\
    \midrule
    RPB  &   1883.32 &    0/ 47 &   58766 \\
    TunedRPB-t   &   1851.83 &    0/ 48 &   58155 \\
    GNN &   1708.99 &    3/ 54 &   39535 \\
    GNN-PAT &    \textbf{1582.39} &   \textbf{57}/ \textbf{59} &   \textbf{39354} \\ \\
    \midrule
    \multicolumn{3}{ c }{Set cover} \\

    \midrule
    FSB  &  917.39 &    9/ 85 &     50 \\
    \midrule
    RPB    &  737.66 &    3/ 92 &    104 \\
    TunedRPB-t   &    751.27 &    5/ 91 &     \textbf{97} \\
    GNN &     \textbf{646.03} &   \textbf{40}/ \textbf{92} &    293 \\
    GNN-PAT &   681.95 &   36/ 91 &    457 \\
    \midrule

    \multicolumn{3}{ c }{facilities} \\

    \midrule
    FSB  &   2700.00 &    0/  0 &     nan \\
    \midrule
    RPB   &   1984.91 &    0/ 32 &   12407 \\
    TunedRPB-t   & 2016.85 &    0/ 33 &   12940 \\
    GNN &   1207.62 &    2/ 65 &    7934 \\
    GNN-PAT &   \textbf{991.54} &   \textbf{70}/ \textbf{72} &    \textbf{6479} \\
    \midrule
    \multicolumn{3}{ c }{indset} \\

    \end{tabular}
    \caption{ }
    \label{tab:results}
\end{table}


==> inputs/cauctions-bigger-side.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{wraptable}{r}{0.65\textwidth}
\vspace{-5pt}
\captionsetup{justification=centering}
\scriptsize
\caption{
Performance of variable selection strategies on \textit{bigger} instances for Combiatorial Auctions instances. See Appendix~\ref{sec:instances} for the instance scaling parameters. 
}
\label{tab:cauctions-bigger}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{8pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=4.0]@{\hspace{3pt}}
    S[table-format=1.6]@{}
%
    }
    \toprule

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Time (c)} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes (c)}  \\ 
    \multicolumn{1}{ c }{Optimality Gap (16)} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{fsb}
        & 2623.50 &  1618.62 &    0 &  5  &    200 &   0.033102 \\

    \cmidrule(lr){1-6} 

    \textsc{rpb}
        & 626.81 & 174.88 &    1 & 80 &   5719 &   0.009555 \\

    \textsc{tunedRPB}
        & 644.20 &  188.22 &    0 & 80 &   6191 &   0.009605 \\
        
    \textsc{gnn}
        & 507.06 & \B 126.94 &   14 & 80 &  \B 5630 &   0.008307 \\

    \textsc{gnn-PAT} (ours)
        & \B 477.26 &  130.72 &  \B 69 & \B 84 &   5757 &   \B 0.007844 \\

    \bottomrule
\end{tabular}

\end{wraptable}


==> inputs/features_G.tex <==
\begin{table}[htb]
    \centering
    \setlength\extrarowheight{-3pt}
    \captionsetup{justification=centering}
    \small
    \caption{Features of $\mathbf{G}$. It is constructed as a variable-constraint bipartite graph, where the vertices of this graph have features as described here. These features are same as used in~\citet{gasse2019exact}.}
    \label{tab:features_G}
    \begin{tabular}{l l p{7cm}}
    \toprule 
     {} & Type & Description \\
    \midrule
    Variable Features (Total -13) & & \\ 
    \midrule
    Variable type (1) & Categorical & Allowed values -  Binary, Integer, Continuous, Implied Integer \\
    Normalized coefficient (1) & Real & Objective coefficient of the variable normalized by the euclidean norm of its coefficients in the constraints  \\
    Specified bounds (2) & Binary & Does the variable has a lower bound (upper bound)? \\ 
    Solution bounds (2) & Binary & If the variable is currently at its lower bound (upper bound)? \\ 
    Solution bractionality (1) & Real $\in [0,1)$ & Fractional part of the variable i.e. $x- \left \lfloor{x}\right \rfloor $, where $x$ is the value of the decision in variable in the current LP solution \\
    Basis (1) & Categorical & One of 4 classes - Lower (variable is at the lower bound), Basic (variable has a value between the bounds), Upper (variable is at the upper bound), Zero (rare case) \\
    Reduced cost (1) & Real & Amount by which objective coefficient of the variable should decrease so that the variable assumes a positive value in the LP solution \\
    Age (1) & Real & Number of LP iterations since the last time the variable was basic normalized by total number of LP iterations \\
    Solution value (1) & Real & Value of the variable in the current LP solution \\ 
    Primal value (1) & Real & Value of the variable in the current best primal solution \\ 
    Average primal value (1) & Real & Average value of the variable in all of the previously observed feasible primal solutions \\ 
    \midrule 
    Constraint Features (Total - 5) \\
    \midrule
    \midrule
    Cossine similarity (1) & Real & Cossine of angle between the vector represented by objective coefficients and the coefficients of this constraint \\
    Bias (1) & Real & Right hand side of the constraint normalized by the euclidean norm of the row coefficients\\
    Age (1) & Real & Number of iterations since the last time the constraint was active normalized by total number of LP iterations  \\
    Normalized dual value (1) & Real & Value of dual variable corresponding to the constraint normalized by the product of norms of the row coefficients and the objective coefficients \\
    Bounds (1) & Binary & If the constraint is currently at its bounds? \\
    \midrule 
    Edge Features (Total - 1)\\ 
    \midrule 
    \midrule
    Normalized coefficient (1) & Real & Coefficient of the variable normalized by the norm of the coefficients of all the variables in the constraint\\
    \bottomrule 
    \end{tabular}
\end{table}


==> inputs/final-results.tex <==
\begin{table}[htp]
    \centering
    \begin{tabular}{p{15mm}|ccc|ccc|ccc}
    \toprule
    {} & \multicolumn{3}{c}{small} & \multicolumn{3}{c}{medium} & \multicolumn{3}{c}{big}\\
    {} & \multicolumn{2}{c}{Time} &  Nodes & \multicolumn{2}{c}{Time} &  Nodes & \multicolumn{2}{c}{Time} &  Nodes \\
    {} &       GM &     Wins &     GM &       GM &     Wins &     GM &  GM &     Wins &     GM  \\
    \midrule
    FSB   &  5.85 &    0/100 &      6 &   127.56 &    0/100 &     72 &   2075.60 &    0/ 53 &    336 \\
    \midrule
    RPB  &   3.89 &    0/100 &     \textbf{11} &    25.31 &    0/100 &    696 &    202.78 &    1/100 &   4640 \\
    TunedRPB  &   3.72 &    0/100 &     \textbf{11} &    24.70 &    0/100 &    \textbf{591} &    205.57 &    0/100 &   4611 \\
    GNN &     \textbf{2.10} &   \textbf{82}/100 &     71 &    \textbf{13.15} &   \textbf{58}/100 &    693 &    \textbf{139.30} &   \textbf{64}/100 &   4142 \\
    GNN-PAT &  2.18 &   18/100 &     72 &    13.25 &   42/100 &    654 &    141.63 &   35/100 &   \textbf{3754} \\
    \bottomrule
    {} & \multicolumn{9}{ c }{Combinatorial Auctions} \\
    
    \midrule
    FSB  &    26.17 &    0/100 &     17 &   531.47 &    0/ 75 &    117 &   2700.00 &    0/  0 &     nan \\
    \midrule
    RPB  &   13.41 &    0/100 &     54 &    91.33 &    0/100 &   1119 &   1883.32 &    1/ 47 &   58766 \\
    TunedRPB   &  13.63 &    0/100 &     \textbf{48} &    93.60 &    0/100 &   1131 &   1851.83 &    0/ 48 &   58155 \\
    GNN &  9.37 &    5/100 &    136 &    64.81 &    1/100 &   1030 &   1708.99 &    5/ 54 &   39535 \\
    GNN-PAT &   \textbf{9.03} &   \textbf{95}/100 &    134 &    \textbf{58.48} &   \textbf{99}/100 &    \textbf{997} &   \textbf{1601.28} &   \textbf{54}/ \textbf{59} &   \textbf{38385} \\
    \midrule
     {} & \multicolumn{9}{ c }{Set Covering} \\

    \midrule
    FSB  &  41.61 &    3/100 &     14 &   264.67 &    3/ 98 &     73 &   917.39 &    8/ 85 &     50 \\
    \midrule
    RPB    &   36.58 &    3/100 &     22 &   206.28 &    1/100 &    147 &   737.66 &    3/ 92 &    104 \\
    TunedRPB   & 37.56 &    1/100 &     \textbf{21} &   211.77 &    2/100 &    \textbf{140} &   751.27 &    2/ 91 &     \textbf{97} \\
    GNN &   \textbf{27.20} &   \textbf{78}/100 &    113 &   146.41 &   \textbf{64}/100 &    320 &   646.03 &   16/ 92 &    293 \\
    GNN-PAT &  29.46 &   15/100 &    112 &   \textbf{159.95} &   30/100 &    329 &   \textbf{581.91} &   \textbf{66}/ \textbf{95} &    304 \\
    \midrule

     {} & \multicolumn{9}{ c }{Capacitated Facility Location} \\

    \midrule
    FSB  & 626.33 &    0/ 93 &     54 &   1634.40 &    0/ 60 &     46 &   2700.00 &    0/  0 &     nan \\
    \midrule
    RPB   & 58.03 &    0/100 &    702 &    144.92 &    0/100 &    770 &   1984.91 &    0/ 32 &   12407 \\
    TunedRPB   & 56.99 &    1/100 &    697 &    143.88 &    2/100 &    \textbf{748} &   2016.85 &    0/ 33 &   12940 \\
    GNN &   35.04 &   28/100 &   1000 &     76.53 &   36/100 &    795 &   1207.62 &   14/ 65 &    7934 \\
    GNN-PAT & \textbf{31.96} &   \textbf{71}/100 &    \textbf{455} &     \textbf{72.00} &   \textbf{62}/100 &    789 &   \textbf{1035.32} &   \textbf{56}/ \textbf{70} &    \textbf{6122} \\
    \midrule
     {} & \multicolumn{9}{ c }{Maximum Independent Set} \\

    \end{tabular}
    \caption{ }
    \label{tab:results}
\end{table}


==> inputs/model-selection-T-15min.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{wraptable}{r}{0.65\textwidth}
\vspace{-5pt}
\captionsetup{justification=centering}
\scriptsize
\caption{
Performance measures on branching strategies selected for facilities instances as per the criteria specified in Eqs.~\ref{eq:b-solved-time} for different time limits $T$ per instance. We observe that the time limit plays an important role in the final models' performance.
}
\label{tab:model-selection-t-15minutes}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{8pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=5.2]@{\hspace{6pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=4.0]@{\hspace{3pt}}
    S[table-format=1.6]@{}
%
    }
    \toprule

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Time (c)} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes}  \\ %&
    \multicolumn{1}{ c }{Optimality Gap (5)} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{gnn}
      &  646.03 & 562.20 &   13 & 92 &    314 & 0.004798  \\
 
    \textsc{gnn-PAT} (Eq.~(\ref{eq:b-solved-time})(T=30mins))
        & \B 581.91 & \B 503.85 &   \B 58 & \B 95  &    \B 326 & \B 0.004070 \\
        
    \textsc{gnn-PAT} (Eq.~(\ref{eq:b-solved-time})(T=15mins)) 
        & 635.04 &  551.53 &   24 & 94 &    388 & 0.006570 \\
    \bottomrule
\end{tabular}
\vspace{-10pt}
\end{wraptable}


==> inputs/other-results.tex <==
\begin{table}[htp]
    \centering
    \begin{tabular}{p{25mm}|ccc|ccc}
    \toprule
    {} & \multicolumn{3}{c}{small} & \multicolumn{3}{c}{medium}\\
    {} & \multicolumn{2}{c}{Time} &  Nodes & \multicolumn{2}{c}{Time} &  Nodes \\
    {} &       GM &     Wins &     GM &       GM &     Wins &     GM \\
    \midrule
    FSB   &  5.85 &    0/100 &      6 &   127.56 &    0/100 &     72  \\
    \midrule
    RPB  &   3.89 &    0/100 &     11 &    25.31 &    0/100 &    696 \\
    TunedRPB-t  &   3.72 &    0/100 &     11 &    24.70 &    0/100 &    591 \\
    GNN &    2.10 &   30/100 &     71 &    13.15 &   25/100 &    693  \\
    GNN-PAT &   \textbf{2.05} &   \textbf{70}/100 &     \textbf{69} &    \textbf{12.33} &   \textbf{75}/100 &    \textbf{648}  \\
    \bottomrule
    \multicolumn{6}{ c }{Combinatorial Auctions} \\
    
    \midrule
    FSB  &    26.17 &    0/100 &     17 &   531.47 &    0/ 75 &    117 \\
    \midrule
    RPB  &   13.41 &    0/100 &     54 &    91.33 &    0/100 &   1119  \\
    TunedRPB-t   &  13.63 &    0/100 &     48 &    93.60 &    0/100 &   1131 \\
    GNN &   9.37 &    1/100 &    136 &    64.81 &    0/100 &   1030 \\
    GNN-PAT &   \textbf{8.60} &   \textbf{99}/100 &    \textbf{133} &    \textbf{55.65} &  100/100 &   \textbf{1000}  \\
    \midrule
    \multicolumn{6}{ c }{Set cover} \\

    \midrule
    FSB  &  41.61 &    3/100 &     14 &   264.67 &    2/ 98 &     73 \\
    \midrule
    RPB    &   36.58 &    3/100 &     22 &   206.28 &    1/100 &    147 \\
    TunedRPB-t   & 37.56 &    1/100 &     \textbf{21} &   211.77 &    0/100 &    \textbf{140}  \\
    GNN &   27.20 &   32/100 &    113 &   \textbf{146.41} &   44/100 &    320  \\
    GNN-PAT &  \textbf{26.94} &   \textbf{61}/100 &    110 &   150.42 &   \textbf{53}/100 &    346 \\
    \midrule

    \multicolumn{6}{ c }{facilities} \\

    \midrule
    FSB  & 626.33 &    0/ 93 &     54 &   1903.22 &    0/ 38 &     52  \\
    \midrule
    RPB   & 58.03 &    0/100 &    702 &    144.92 &    0/100 &    770 \\
    TunedRPB-t   & 56.99 &    2/100 &    697 &    143.88 &    1/100 &    748 \\
    GNN &   35.04 &    8/100 &   1000 &     76.53 &   14/100 &    795 \\
    GNN-PAT & \textbf{30.62} &   \textbf{90}/100 &    \textbf{620} &     \textbf{63.02} &   \textbf{85}/100 &    \textbf{593}  \\
    \midrule
    \multicolumn{6}{ c }{indset} \\

    \end{tabular}
    \caption{ }
    \label{tab:results}
\end{table}


==> inputs/results_template.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[t]
\caption{
Performance of \textit{branching strategies} on evaluation instances. We report geometric mean of solving times, number of times a method won (in solving time) over total finished runs, and geometric mean of number of nodes. Refer to section~\ref{sec:experiments} for more details. The best performing results are in \textbf{bold}. $^*$Models were regularized to prevent overfitting on small instances.}
\label{tab:evaluation}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{10pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=3.2]@{\hspace{10pt}}
    S[table-format=2.0]@{\hspace{4pt}/\hspace{-4pt}}
    S[table-format=2.0]@{\hspace{5pt}}
    S[table-format=3.0]@{}
%
    S[table-format=3.2]@{\hspace{10pt}}
    S[table-format=2.0]@{\hspace{4pt}/\hspace{-4pt}}
    S[table-format=2.0]@{\hspace{5pt}}
    S[table-format=3.0]@{}
%
    S[table-format=3.2]@{\hspace{10pt}}
    S[table-format=2.0]@{\hspace{4pt}/\hspace{-4pt}}
    S[table-format=2.0]@{\hspace{5pt}}
    S[table-format=3.0]@{}
    }
    \toprule
     &
    \multicolumn{4}{ c }{Small} &
    \multicolumn{4}{ c }{Medium} &
    \multicolumn{4}{ c }{Big} \\

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{2}{ c }{Wins} &
    \multicolumn{1}{ c }{Nodes} &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{2}{ c }{Wins} &
    \multicolumn{1}{ c }{Nodes} &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{2}{ c }{Wins} &
    \multicolumn{1}{ c }{Nodes} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{fsb}
        &   42.53 &   1 &  60 &   13
        &  313.33 &   0 &  59 &   75
        &  997.23 &   0 &  51 &   50  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \textsc{rpb}
        &   36.86 &   1 &  60 &  \B  23
        &  213.99 &   1 &  60 &  \B 152
        &  794.80 &   2 &  54 &  \B 99 \\

    \textsc{tunedRPB}
        &   30.37 &   3 &  60 & 120 
        &  172.51 &   4 &  60 & 347 
        &  633.42 &   6 &  57 & 294  \\

    \textsc{gnn}
        &   39.18 &   0 & 60 &  112 
        &  209.84 &   0 & 60 &  314 
        &  748.85 &   0 & 54 &  286 \\

    \textsc{FiLM} (ours)
        & \B   24.67 & \B  51 &  60 &  109 
        & \B  136.42 & \B  51 &  60 &  325
        & \B  531.70 & \B  46 &  57 &  295  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{gnn-gpu}
        &      28.91 &     \text{--} &  60 &  112 
        &     150.11 &     \text{--} &  60 &  314
        &     628.12 &     \text{--} &  56 &  286  \\
        
    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \\[-7pt]
    & \multicolumn{12}{ c }{Capacitated Facility Location} \\
    \\[-3pt]

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \textsc{fsb}
        &   27.16 &    0 &  60 & 17
        &  582.18 &    0 &  45 & 116 
        & 2700.00 &    0 &   0 & n/a  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{pb}
        &   10.19 &   0 &  60 & 286
        &   94.12 &   0 &  60 & 2451
        & 2208.57 &   0 &  23 & 82624  \\

    \textsc{rpb}
        &   14.05 &    0 &  60 & \B     54
        &   94.65 &    0 &  60 & 1129
        & 1887.70 &    7 &  27 & 48395 \\

    \textsc{comp}
        &    9.83 &   3 &  60 & 178
        &   89.24 &   0 &  60 & 1474
        & 2166.44 &   0 &  21 & 52326  \\

    \textsc{gnn}
        &   17.61 &   0 &  60 & 136
        &  242.15 &   0 &  60 & \B  1013
        & 2700.17 &   0 &   0 & n/a \\

    \textsc{FiLM} (ours)
        & \B    8.73 & \B 57 &     60 & 147
        & \B   63.75 & \B 60 &     60 & 1131
        & \B 1843.24 & \B 20 &     26 & \B  37777 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{gnn-gpu}
        &       8.26 &     \text{--} &  60 &  136
        &      53.56 &     \text{--} &  60 &  1013
        &    1535.80 &     \text{--} &  36 &  31662  \\
    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \\[-7pt]
    & \multicolumn{12}{ c }{Set Covering} \\
    \\[-3pt]


    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \textsc{fsb}
        &    6.12 &    0 &  60 & 6
        &  132.38 &    0 &  60 & 71
        & 2127.35 &    0 &  28 & 318  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{pb}
        &    2.76 &   1 &  60 & 234
        &   25.83 &   0 &  60 & 2765
        &  393.60 &   0 &  59 & 13719  \\

    \textsc{rpb}
        &    4.01 &       0 &  60 & \B 11
        &   26.36 &       0 &  60 & 714
        &  \B 210.95 & \B   29 &  60 & 4701 \\

    \textsc{comp}
        &    2.76 &   0 &  60 & 82
        &   29.76 &   0 &  60 & 930
        &  494.59 &   0 &  54 & 5613  \\

    \textsc{gnn}
        &    2.73 &   1 &  60 & 71
        &   22.26 &   0 &  60 & 688
        &  257.99 &   6 &  60 & \B 3755 \\

    \textsc{FiLM} (ours)
        & \B    2.13 & \B 58 &     60 & 73
        & \B   15.71 & \B 60 &     60 &\B  686
        &     217.02 &    25 &     60 &  4315 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{gnn-gpu}
        &       1.96 &     \text{--} &  60 &  71
        &      11.70 &     \text{--} &  60 &  688
        &     121.18 &     \text{--} &  60 &  3755  \\
    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \\[-7pt]
    & \multicolumn{12}{ c }{Combinatorial Auctions} \\
    \\[-3pt]

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}

    \textsc{fsb}
        &  673.43 &    0 &  53 & 47
        & 1689.75 &    0 &  20 & 10
        & 2700.00 &    0 &   0 & n/a  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{pb}
        &  172.03 &   2 &  57 & 5728
        &  753.95 &   0 &  45 & 1570
        & 2685.23 &   0 &   1 & 38215  \\

    \textsc{rpb}
        &   59.87 &       5 &  60 & 603
        &  173.17 &      11 &  60 & \B 205
        & 1946.51 &       9 &  21 & 2461 \\

    \textsc{comp}
        &   82.22 &  1 &  58 & 847
        &  383.97 &  1 &  52 & 267
        & 2393.75 &  0 &   6 & 5589  \\

    \textsc{gnn$^\star$}
        &\B 44.07 &  15 &  60 & \B 331
        &  625.23 &   1 &  50 & 599
        & 2330.95 &   0 &  10 & \B 687 \\

    \text{FiLM$^\star$} (ours)
        &      52.96 & \B 37 &     55 & 376
        & \B  131.45 & \B 47 &     54 & 264
        & \B 1823.29 & \B 12 &     15 &  1201 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    \textsc{gnn-gpu$^\star$}
        &      31.71 &     \text{--} &  60 &  331
        &      63.96 &     \text{--} &  60 &  599
        &    1158.59 &     \text{--} &  27 &  685  \\
        
    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    % \bottomrule
    \\[-7pt]
     & \multicolumn{12}{ c }{Maximum Independent Set} \\
     \bottomrule
\end{tabular}
\vspace{-15pt}
\end{table}


==> inputs/small-medium-scip.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[!ht]
\caption{
Performance of \textit{branching strategies} on evaluation instances. In this table, we include default SCIP and TunedSCIP. We report geometric mean of solving times, number of times a method won (in solving time) over total finished runs, and geometric mean of number of nodes. Refer to section~\ref{sec:experiments} for more details. The best performing results are in \textbf{bold}.}
\label{tab:small-medium-evaluation-scip}
\centering
% \footnotesize
\scriptsize
\setlength{\tabcolsep}{8pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm \;\;\;\;\;\;
\begin{tabular}{
    c
    S[table-format=4.2]@{\hspace{6pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=3.0]@{}
%
    S[table-format=4.2]@{\hspace{10pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=2.0]@{\hspace{3pt}}
    S[table-format=3.0]@{}
%
    }
    \toprule
     &
    \multicolumn{4}{ c }{Small} &
    \multicolumn{4}{ c }{Medium} \\
    % \multicolumn{4}{ c }{Big} \\

    Model &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes} &
    \multicolumn{1}{ c }{Time} &
    \multicolumn{1}{ c }{Wins} &
    \multicolumn{1}{ c }{Solved} &
    \multicolumn{1}{ c }{Nodes} \\
    \toprule

    % \cmidrule{1-13}

    \textsc{fsb}
        &  5.85   &   0 & 100 &   6 
        &  127.56 &   0 & 100 &  72 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}

    \textsc{rpb}
        &  3.89  &   0 & 100 &   11
        &  25.31 &   0 & 100 &    696 \\ 

    \textsc{tunedRPB}
        &   3.72  &   0 & 100 &  11
        &  24.70 &    0 & 100 &  \B 591 \\

    \textsc{scip}
        &   6.13 &    0 & 100 &     \B 8
        &  25.55 &    0 & 100 &    639 \\

    \textsc{tunedscip}
        &  \B 1.88 &   \B 63 & 100 &     21
        &  18.14 &    1 & 100 &    780  \\


    \textsc{gnn}
        & 2.10  &  33  & 100 &   71
        & \B 13.15 &  \B 58  & 100 &  693 \\ 

    \textsc{gnn-PAT} (ours)
        &  2.18  &   4  & 100 &  72
        &  13.25 &   41  & 100 & 654  \\ 

       
    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    \\[-7pt]
    & \multicolumn{8}{ c }{Combinatorial Auction} \\
    \\[-3pt]

    \cmidrule(lr){1-5} \cmidrule(lr){6-9} \\

    \textsc{fsb}
        &   26.17 &    0 & 100 &  17
        &  531.47 &    0 & 75  &  117 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}

    \textsc{rpb}
        &  13.41 &   0 & 100 &     54
        &  91.33 &   0 & 100 &   1119 \\

    \textsc{tunedRPB}
        &  13.63 &   0 & 100 &  \B 48 
        &  93.60 &   0 & 100 &   1131 \\

    \textsc{scip}
        &   18.52 &    0 & 100 &     63
        &   90.60 &    0 & 100 &    1109 \\

    \textsc{tunedscip}
        & \B 4.30 &  \B 100 & 100 &     78
        & \B 49.01 & \B  97 & 100 &    1130  \\

    \textsc{gnn}
        &  9.37  &   0 & 100 &    136
        &  64.81 &   0 & 100 &   1030  \\ 

    \textsc{gnn-PAT} (ours)
        & 9.03  &   0 & 100 &    134 
        & 58.48 &   3 & 100 &  \B 997 \\ 

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    \\[-7pt]
    & \multicolumn{8}{ c }{Set Covering} \\
    \\[-3pt]


    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    
    \textsc{fsb}
        &   41.61 &  3 & 100 &     14
        &  264.67 &  3 &  98 &     73 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}

    \textsc{rpb}
        &  36.58 &   0 & 100 &     22 
        &  206.28 &  1 & 100 &    147 \\

    \textsc{tunedRPB}
        &  37.56 &   0 & 100 &  21
        &  211.77 &  2 & 100 &  140 \\ 

    \textsc{scip}
        &   35.27 &    4 & 100 &    \B 14
        &   185.21 &  8 & 100 &  \B  108 \\

    \textsc{tunedscip}
        & 27.37 &  27 & 100 &     23
        & 171.00 &  17 & 100 &    124  \\

    \textsc{gnn}
        &  \B 27.20 &   \B 60 & 100 & 113
        &  \B 146.41 &   \B 52 & 100 & 320  \\

    \textsc{gnn-PAT} (ours)
        & 29.46    &   8 & 100 &    112 
        & 159.95 &   19 & 100 &    329 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    \\[-7pt]
    & \multicolumn{8}{ c }{Capacitated Facility Location} \\
    \\[-3pt]


    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    
    \textsc{fsb}
        &   626.33 &   0 & 93 &     54 
        &  1634.40 &  0 & 60 &     46 \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}

    \textsc{rpb}
        &  58.03 &   0 & 100 &    702 
        &  144.92 &  0 & 100 &    770 \\

    \textsc{tunedRPB}
        &  56.99 &  0 & 100 &    697
        &  143.88 & 1 & 100 &    \B 748 \\

    \textsc{scip}
        &   57.18 &   0 & 100 &   702
        &  138.92 &   0 & 100 &   770 \\

    \textsc{tunedscip}
        & 49.13 &  4 & 100 & 821
        & 125.14 & 3 & 100 & 1160  \\

    \textsc{gnn}
        &  35.04 &   28 & 100 &  1000
        &  76.53 &   36 & 100 &  795 \\

    \textsc{gnn-PAT} (ours)
        & \B 31.96 &   \B 68 & 100 &    \B 455
        & \B 72.00 &   \B 60 & 100 & 789  \\

    \cmidrule(lr){1-5} \cmidrule(lr){6-9}
    \\[-7pt]
    & \multicolumn{8}{ c }{Maximum Independent Set} \\
     \bottomrule
\end{tabular}
\vspace{-15pt}
\end{table}

